Making "fetch" happen: The influence of social and linguistic context on nonstandard word growth and decline

In an online community, new words come and go: today's "haha" may be replaced by tomorrow's "lol." Changes in online writing are usually studied as a social process, with innovations diffusing through a network of individuals in a speech community. But unlike other types of innovation, language change is shaped and constrained by the system in which it takes part. To investigate the links between social and structural factors in language change, we undertake a large-scale analysis of nonstandard word growth in the online community Reddit. We find that dissemination across many linguistic contexts is a sign of growth: words that appear in more linguistic contexts grow faster and survive longer. We also find that social dissemination likely plays a less important role in explaining word growth and decline than previously hypothesized.

==> cox-regression-deviance-table.tex <==
\begin{tabular}{l l l l l}
  \toprule
Model & Deviance & d.f. & $\chi^{2}$ & $p$-value \\ \midrule
Null & 4383 & 0 & ~ & ~ \\ 
\model{f} & 4375 & 1 & 16.19 & *** \\ 
\model{f+S} & 4370 & 4 & 27.24 & *** \\ 
\model{f+L} & 4337 & 2 & 93.32 & *** \\ 
\model{f+L+S} & 4331 & 5 & 103.8 & *** \\ 
\bottomrule
%output/cox_regression_deviance_output.txt
\end{tabular}

==> pred-table.tex <==
\begin{tabular}{l r r r r}
\toprule
  Predictor & \multicolumn{1}{l}{$\mu_{\beta}$} & \multicolumn{1}{l}{$\sigma_{\beta}$} & \multicolumn{1}{l}{$t$} & \multicolumn{1}{l}{$p$} \\ \midrule
const & -0.4935 & 0.3223 & -1.531 & ~ \\
$\var{f}$ & 0.4393 & 0.0651 & 6.748 & *** \\
$\var{D^{C}}$ & 3.824 & 0.3907 & 9.786 & *** \\
$\var{D^{U}}$ & 3.287 & 0.6079 & 5.407 & *** \\
$\var{D^{S}}$ & 1.940 & 0.3784 & 5.127 & *** \\
$\var{D^{T}}$ & -0.7693 & 0.5997 & -1.283 & ~ \\
\bottomrule
\end{tabular}

